A Tale of Two Linkings: Dynamically Gating between Schema Linking and Structural Linking for Text-to-SQL Parsing

In Text-to-SQL semantic parsing, selecting the correct entities (tables and columns) for the generated SQL query is both crucial and challenging; the parser is required to connect the natural language (NL) question and the SQL query to the structured knowledge in the database. We formulate two linking processes to address this challenge: schema linking which links explicit NL mentions to the database and structural linking which links the entities in the output SQL with their structural relationships in the database schema. Intuitively, the effectiveness of these two linking processes changes based on the entity being generated, thus we propose to dynamically choose between them using a gating mechanism. Integrating the proposed method with two graph neural network-based semantic parsers together with BERT representations demonstrates substantial gains in parsing accuracy on the challenging Spider dataset. Analyses show that our proposed method helps to enhance the structure of the model output when generating complicated SQL queries and offers more explainable predictions.

==> Makefile <==
### latex.makefile
# Author: Jason Hiebel

PROJECT = main

# This is a simple makefile for compiling LaTeX documents. The core assumption
# is that the resulting documents should have any parameters effecting
# rendering quality set to theoretical limits and that all fonts should be
# embedded. While typically overkill, the detriment to doing so is negligible.

# Targets:
#    default : compiles the document to a PDF file using the defined
#              latex generating engine. (pdflatex, xelatex, etc)
#    display : displays the compiled document in a common PDF viewer.
#              (currently linux = evince, OSX = open)
#    clean   : removes the obj/ directory holding temporary files

default: obj/$(PROJECT).pdf

display: default
	(${PDFVIEWER} obj/$(PROJECT).pdf &)


### Compilation Flags
PDFLATEX_FLAGS  = -halt-on-error -output-directory obj/

TEXINPUTS = .:obj/
TEXMFOUTPUT = obj/


### File Types (for dependancies)
TEX_FILES = $(shell find . -name '*.tex' -or -name '*.sty' -or -name '*.cls')
BIB_FILES = $(shell find . -name '*.bib')
BST_FILES = $(shell find . -name '*.bst')
IMG_FILES = $(shell find . -path '*.jpg' -or -path '*.png' -or \( \! -path './obj/*.pdf' -path '*.pdf' \) )


### Standard PDF Viewers
# Defines a set of standard PDF viewer tools to use when displaying the result
# with the display target. Currently chosen are defaults which should work on
# most linux systems with GNOME installed and on all OSX systems.

UNAME := $(shell uname)

ifeq ($(UNAME), Linux)
PDFVIEWER = evince
endif

ifeq ($(UNAME), Darwin)
PDFVIEWER = open
endif


### Clean
# This target cleans the temporary files generated by the tex programs in
# use. All temporary files generated by this makefile will be placed in obj/
# so cleanup is easy.

clean::
	rm -rf obj/

### Core Latex Generation
# Performs the typical build process for latex generations so that all
# references are resolved correctly. If adding components to this run-time
# always take caution and implement the worst case set of commands.
# Example: latex, bibtex, latex, latex
#
# Note the use of order-only prerequisites (prerequisites following the |).
# Order-only prerequisites do not effect the target -- if the order-only
# prerequisite has changed and none of the normal prerequisites have changed
# then this target IS NOT run.
#
# In order to function for projects which use a subset of the provided features
# it is important to verify that optional dependancies exist before calling a
# target; for instance, see how bibliography files (.bbl) are handled as a
# dependency.

obj/:
	mkdir -p obj/

obj/$(PROJECT).aux: $(TEX_FILES) $(IMG_FILES) | obj/
	pdflatex $(PDFLATEX_FLAGS) $(PROJECT)

obj/$(PROJECT).bbl: $(BIB_FILES) | obj/$(PROJECT).aux
	bibtex obj/$(PROJECT)
	pdflatex $(PDFLATEX_FLAGS) $(PROJECT)

obj/$(PROJECT).pdf: obj/$(PROJECT).aux $(if $(BIB_FILES), obj/$(PROJECT).bbl)
	pdflatex $(PDFLATEX_FLAGS) $(PROJECT)


==> mydef.tex <==
%% Based on Jacob's mystuff-nlp.sty
%% Modified by Yangfeng Ji

\usepackage{amsmath,amsfonts,amssymb,bm}
\usepackage{pifont} % http://ctan.org/pkg/pifont
\usepackage{graphicx,subfigure,epsfig,fancybox} % figures & graph
\usepackage{float}
\usepackage{color} % color
% \usepackage[]{algorithm2e} %
\usepackage{multirow}
\usepackage{natbib}

%% -----------------
%% Tikz
\usepackage{tikz}
\usetikzlibrary{shapes.geometric, positioning, calc}
\usetikzlibrary{arrows,shapes,calc}
\usetikzlibrary{trees,positioning,mindmap,shadows,fit}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{tikzmark} % for annotating tables
\usetikzlibrary{intersections} % for pyramid


\newcommand{\mycite}[1]{\small{(#1)}}
\newcommand{\revised}[1]{\textcolor{blue}{}}
\renewcommand{\vec}[1]{\boldsymbol{#1}}
\newcommand{\eq}[1]{\left\langle #1 \right\rangle}
\newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\trans}[1]{#1^{\textsf{T}}}
\newcommand{\Count}[1]{\text{count}(#1)}
\newcommand{\inv}[1]{(#1)^{-1}}
\newcommand{\Inv}[1]{\left(#1\right)^{-1}}
\newcommand{\set}[1]{\mathcal{#1}}
\newcommand{\diag}[1]{\text{diag}\left(#1\right)}
\newcommand{\annotation}[1]{\textsc{#1}}
\newcommand{\annot}[1]{\annotation{#1}}
\newcommand{\tagword}[2]{\example{#1}/\annot{#2}}
\newcommand{\phon}[1]{\textsf{#1}}
% \newcommand{\argmax}[1]{\text{arg}\max_{#1}}
% \newcommand{\argmin}[1]{\text{arg}\min_{#1}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\expect}[1]{E[{#1}]}
\newcommand{\dd}[2]{\frac{\partial #1}{\partial #2}}
\renewcommand{\symbol}[1]{$\langle$#1$\rangle$}
\newcommand{\sentstart}[0]{\symbol{s}}
\newcommand{\sentend}[0]{\symbol{/s}}
\newcommand{\tuple}[1]{\langle #1 \rangle}
\newcommand{\cue}[1]{[\textcolor{blue}{#1}]}
\newcommand{\question}[1]{\textcolor{red}{#1}}
\newcommand{\fstransx}[2]{\xrightarrow[\example{#2}]{\example{#1}}}
\newcommand{\fstrans}[2]{\xrightarrow[{#2}]{#1}}
\newcommand{\gloss}[1]{{\fontfamily{phv}\selectfont #1}}
\newcommand{\newadd}[1]{\textcolor{magenta}{#1}}

\newcommand{\from}[0]{\leftarrow}
\newcommand{\reals}[0]{\mathbb{R}}
\newcommand{\normal}[1]{\mathcal{N}\left(#1\right)}
\newcommand{\cpic}[2][.95\textwidth]{\begin{center}\includegraphics[width=#1]{#2}\end{center}}
% \newcommand{\etal}[0]{\textit{et al.}~}
\newcommand{\bigo}[1]{\mathcal{O}(#1)}
\newcommand{\Pmult}[0]{P_{\text{multinomial}}}
\newcommand{\Pcat}[0]{P_{\text{categorical}}}
\newcommand{\vw}[0]{\vec{w}}
\newcommand{\vwt}[0]{\trans{\vec{w}}}
\newcommand{\vd}[0]{\vec{d}}
\newcommand{\vf}[0]{\vec{f}}
\newcommand{\vx}[0]{\vec{x}}
\newcommand{\vz}[0]{\vec{z}}
\newcommand{\vy}[0]{\vec{y}}
\newcommand{\vs}[0]{\vec{s}}
\newcommand{\vu}[0]{\vec{u}}
\newcommand{\vth}[0]{\vec{\theta}}
\newcommand{\vtht}[0]{\trans{\vec{\theta}}}
\newcommand{\vph}[0]{\vec{\phi}}
\newcommand{\jm}[0]{J\&M}
\newcommand{\dkl}[0]{\mathcal{D}_{KL}}
\newcommand*{\defeq}{\mathrel{\vcenter{\baselineskip0.5ex \lineskiplimit0pt\hbox{\scriptsize.}\hbox{\scriptsize.}}}=}
\newcommand{\refeq}[1]{(\ref{#1})}

\newenvironment{exampleenv}{\rmfamily}{\normalfont}

\newcommand{\myaddress}[0]{
  Yangfeng Ji\\
  College of Computing, School of Interactive Computing\\
  85 5th Street NW, Atlanta, Georgia 30332\\
  Email: jiyfeng@gatech.edu
}
\newcommand{\gatech}[0]{Georgia Institute of Technology}
\usepackage{adjustbox}
\usepackage{array}
\usepackage{booktabs}

\newcolumntype{R}[2]{%
    >{\adjustbox{angle=#1,lap=\width-(#2)}\bgroup}%
    l%
    <{\egroup}%
}
\newcommand*\rot{\multicolumn{1}{R{45}{0.4em}}}

%% ****************************************************
%% Editing labels
%% Added by Yangfeng Ji
% \usepackage{trackchanges}
% \newcommand{\yfnote}[1]{\note[YJ]{#1}}
% \usepackage[disable]{todonotes}
\usepackage{todonotes}
\usepackage{setspace}
\newcommand{\yfnote}[1]{\todo[color=green]{\begin{singlespace}\scriptsize{YJ: #1}\end{singlespace}}} % [color=green!40]
\newcommand{\yfcomment}[1]{[\textcolor{blue}{\tt #1 - YJ}]}
\newcommand{\xiaodl}[1]{[\textcolor{green}{\tt #1 - XDL}]}

\newcommand{\here}{\textcolor{red}{\tt It ends here last time.}}

%% -----------------
%% Misc
\def\etal{{\it et~al.}}


